Probing the flavor dependence of proton's light-quark sea in the SeaQuest experiment

Surprisingly large flavor asymmetry of the light-quark sea in the proton was reported in deep-inelastic scattering and Drell-Yan experiments. The Bjorken-$x$ dependence of the $\bar{d}/\bar{u}$ ratio extracted from the Fermilab E866 experiment also revealed an intriguing drop at the highest values of $x$. The Fermilab E906/SeaQuest experiment was designed to measure $\bar{d}/\bar{u}$ with improved accuracy at high Bjorken-$x$. By detecting high-mass dimuon events produced in the interaction of 120 GeV proton beam with liquid hydrogen (LH$_2$) and deuterium (LD$_2$) targets, the SeaQuest experiment probes the $\bar{d}/\bar{u}$ ratio up to $x \approx 0.45$. Data collection has been completed and we report the status of data analysis for SeaQuest. Two different methods for extracting the LD$_2$/LH$_2$ Drell-Yan cross section ratios for $0.1\leq x\leq 0.45$ are discussed. These ratios are compared with calculations using various PDFs.

==> Sections/CSR.tex <==
\section{Comparison with E866}

The E906 and E866 data agree in the low $x$ region, where the statistics of the E866 experiment were high.  However, E906 shows a cross section ratio consistent with remaining above 1 for all $x$.  Above $x$ of 0.2, E866 begins to suffer from poor statistics and drops below unity.  E866 computer their cross section ratio for three separate mass ranges and combined the result.  It has been shown that when averaging multiple ratios if Poissonian statistics are not properly considered, the average will be lower than simply taking the ratio of the combined data.  It is believed that this is one of the causes for the  drop in the E866 ratio at high $x$.

\begin{figure}[H]
\centering
\includegraphics[scale=0.4]{Images/E906_E866_only.pdf}
\caption{Comparison of E906 cross section ratio with E866.  The data is not directly comparable due to differing acceptance, beam energy, and $x_1$ distributions.  The discrepancy between experiments above $x_2>0.2$ is likely due to a combination of statistics and acceptance edge effects for E866.  The systematics for E866 are less than 1\% and are not shown.}
\label{fig:E906_E866}
\end{figure}


==> Sections/Motivation.tex <==
\section{Motivation}
\subsection{Violation of Gottfried Sum Rule}
Perturbation theory suggests that momentum of sea quarks which arise from gluon splitting should be flavor independent.  In the 1980's the NMC experiment at CERN measured a violation the Gottfried sum rule which was the first experimental evidence for a flavor asymmetry.  The Gottfried sum rule states

\begin{equation}
    S_G = \int_0^1 (F_2^p-F_2^n)\frac{dx}{x} = \frac{1}{3}+\frac{2}{3}\int_0^1[\bar{u}^p(x)-\bar{d}^p(x)]dx
\end{equation}

Given a symmetric sea, one would expect $S_G=1/3$.  The measurement reported the integral from $0.004 < x < 0.8$ as $S_G=0.235\pm 0.026$.  While indicative of a flavor asymmetric sea, it still left open the possibility of pathological behavior in the unmeasured regions of $x$.


\subsection{Flavor Asymmetry as a Function of $x$}

Later, the NA51 and E866 experiments used the Drell-Yan procedure to more directly measure the asymmetry.  Unlike DIS, Drell-Yan directly probes the antiquarks in one of the colliding hadrons.  This allows the flavor asymmetry, $\bar{d}/\bar{u}$, to be measured as a function of $x$.


\begin{figure}[H]
\centering
\includegraphics[scale=0.4]{Images/E866Ratio.png}
\caption{NA51 and E866 measurement of $\bar{d}/\bar{u}$ \cite{E866_01}.  Systematic uncertainty is included for the E866 data.  Parametrizations of various PDFs are compared with the data.}
\label{fig:E866Ratio}
\end{figure}

While some of the models were able to explain the $\bar{d}>\bar{u}$ asymmetry at low $x$, none of the models could reproduce $\bar{d}<\bar{u}$.  The E906 experiment was developed to help resolve the poor statistics in the region $x>0.2$.
